Estimating Mixture Models via Mixtures of Polynomials

Mixture modeling is a general technique for making any simple model more expressive through weighted combination. This generality and simplicity in part explains the success of the Expectation Maximization (EM) algorithm, in which updates are easy to derive for a wide class of mixture models. However, the likelihood of a mixture model is non-convex, so EM has no known global convergence guarantees. Recently, method of moments approaches offer global guarantees for some mixture models, but they do not extend easily to the range of mixture models that exist. In this work, we present Polymom, an unifying framework based on method of moments in which estimation procedures are easily derivable, just as in EM. Polymom is applicable when the moments of a single mixture component are polynomials of the parameters. Our key observation is that the moments of the mixture model are a mixture of these polynomials, which allows us to cast estimation as a Generalized Moment Problem. We solve its relaxations using semidefinite optimization, and then extract parameters using ideas from computer algebra. This framework allows us to draw insights and apply tools from convex optimization, computer algebra and the theory of moments to study problems in statistical estimation.

==> experiments.tex <==
%%%\vspace{-1.5em}
\section{Experiments}
%%%\vspace{-0.5em}
\label{sec:experiments}
We implemented a GMP solver and several mixture models
(code: \url{http://annon}) in Python.
We used CVXOPT to handle the SDP, and the random projections algorithm
from Section~\ref{sec:solution-extraction}
to extraction solutions.
In \tableref{experiments}, we show the relative error
$\max_k  || \prm\ind{k} - \prmt\ind{k} ||_2 / ||\prmt\ind{k} ||_2$
averaged over 10 random models of each class.
\newcommand{\first}[1]{\textbf{#1}}
\newcommand{\sketchy}[1]{\sout{#1}}
%%\vspace{-1em}
\begin{table}
\centering
\begin{tabular}{|l|l|lll|lll|lll|}
   &         \textbf{ Methods}  &  EM&TF&Poly&       EM& TF&Poly&       EM&TF&Poly\\
\hhline{-----------}
\textbf{Models} &$K,D$& \multicolumn{3}{c|}{$T=10^3$} & \multicolumn{3}{c|}{$T=10^4$} & \multicolumn{3}{c|}{$T=10^5$} \\
\hhline{-----------}
spherical Gaussian  & $2,2$ &
\first{0.37} & 2.05 & 0.58 &
\first{0.24} & 0.73 & 0.29 &
0.19 & 0.36 & \first{0.14} \\
% Diagonal Gaussian (rotated) & % hmm, TF did not work at all, not sure if thats fair
% 0.89 &  9.11& 0.57&
% 0.92 & 38 & 0.51&
% 0.79 & 10.85 & 0.5\\
diagonal Gaussian&  $2,2$  &        
\first{0.44} & \sketchy{2.15} & 0.48 &
0.48 & \sketchy{4.03} & \first{0.40} &
0.38 & \sketchy{2.46} & \first{0.35} \\
constrained Gaussian  &   $2,2$     &
0.49 & \sketchy{7.52} & \first{0.38} &
0.47 & \sketchy{2.56} & \first{0.30} &
0.34 & \sketchy{3.02} & \first{0.29} \\
\hhline{===========}
\textbf{Models} & $K,D$& \multicolumn{3}{c|}{$T=10^4$} & \multicolumn{3}{c|}{$T=10^5$} & \multicolumn{3}{c|}{$T=10^6$} \\
\hhline{-----------}
3-view multinomial&  $3,3$ &
\first{0.38}&0.51&0.57&          
0.31&0.33&\first{0.26}&              
0.36&0.16&\first{0.12} \\
linear regression &     $2,2$ &     
-&-&\first{3.51}&                
-&-&\first{2.60}&                 
-&-&\first{2.52} \\
%Constrained Multiview?  &           -&-&?&           -&-&?&             -&-&?      \\
%\hhline{-----------}
\end{tabular}
\caption{$T$ is the number of samples, and the error metric is defined above.
\textbf{Methods:}
EM\@: sklearn initialized with k-means using 5 random restarts;
TF\@: tensor power method implemented in Python;
Poly\@: Polymom by solving \problemref{gmpsdp}.
\textbf{Models:} for mixture of Gaussians, we have
$\sigma \approx 2 || \mu_1 - \mu_2 ||_2$; 'spherical' and 'diagonal'
describes the type of covariance matrix.
The mean parameters of constrained Gaussians satisfies $\mu_1 + \mu_2 = 1$.
The best result is \first{bolded}. 
TF only handles spherical variance, but it was of interest to
see what TF does if the data is drawn from mixture of Gaussians with
diagonal covariance, these results are in \sketchy{strikeout}.
}
\label{tbl:experiments}
\end{table}
%\pl{show that being able to incorporate constraints (non-negativity, parameter tying) helps, oh well, doesnt really help in these cases, unfortunately}



==> figures/macros.tex <==
\newif\ifshowcomments
%\showcommentstrue
\ifshowcomments
\newcommand\ac[1]{\textcolor{red}{[AC: #1]}}
\newcommand\pl[1]{\textcolor{red}{[PL: #1]}}
\newcommand\pled[1]{\textcolor{orange}{[PL(done): #1]}}
\newcommand\sidaw[1]{\textcolor{green}{[sidaw: #1]}}
\else
\newcommand\ac[1]{}
\newcommand\pl[1]{}
\newcommand\pled[1]{}
\newcommand\sidaw[1]{}
\fi

% \usepackage{scalerel}
% \DeclareMathOperator*{\Bigcdot}{\scalerel*{\cdot}{\bigodot}}
\providecommand{\bigcdot}{\bullet}

\providecommand{\ind}[1]{_{#1}} % of (t) 
\providecommand{\inds}[2]{_{#1,#2}} % of (t) with additional stuff

\providecommand{\xt}{{\bar{x}}} % True parameter (x true)
\providecommand{\mt}{{\bar{m}}} % true vector of basis  (bold b true)
\providecommand{\byt}{{\by^*}} % True moment parameter vector
                                % (bold y true)
\providecommand{\byh}{\hat{\by}} % recovered moment (vector bold y hat)

\providecommand{\bbt}{{\bar{\bb}}} % true vector of basis  (bold b true)
\providecommand{\bmt}{{\bar{\bm}}} % true vector of basis  (bold b true)
\providecommand{\balpha}{{\boldsymbol\alpha}} % bold alpha
\providecommand{\bbeta}{{\boldsymbol\beta}} % bold beta
\providecommand{\bgamma}{{\boldsymbol\gamma}} % bold gamma
\providecommand{\bVt}{{\bV^*}}
\providecommand{\KK}{\mathbb{K}}

\renewcommand{\Re}{\mathbb{R}} % real number that i like better
\providecommand{\RR}{\mathbb{R}} % backwards compatible
\providecommand{\NN}{\mathbb{N}} % non-neg integers
\providecommand{\Lo}{\mathcal{L}} % the linear operator
\providecommand{\Loy}{\mathscr{L}_{\by}} % the linear operator
\providecommand{\Mea}{\mathcal{M}} % the set of measures
\providecommand{\MM}{\mathbf{M}} % the moment matrix
\providecommand{\MMh}{\hat{\mathbf{M}}} % the noisy moment matrix
\providecommand{\coeff}[2]{a_{#1#2}}

%%%%% Symbols for parameters and data %%%%%%%%%
\providecommand{\sprm}{\theta} % scalar paramete
\providecommand{\sprmt}{\sprm^*} % scalar parameter true
\providecommand{\sprmh}{\hat{\sprm}} % parameters true

\providecommand{\prm}{{\boldsymbol\sprm}} % parameters
\providecommand{\prmt}{\prm^*} % parameters true

\providecommand{\prmh}{\hat{\prm}} % parameters true
\providecommand{\allprm}{[\prm_k]_{k=1}^K} % all parameters
\providecommand{\allprmt}{[\prmt_k]_{k=1}^K} % all parameters true
\providecommand{\alldat}{\bX} % data
\providecommand{\dat}{\bx} % data vector
\providecommand{\sdat}{x} % scalar data

\providecommand{\Cmpn}{A} % letter for the multiplication matrix

\providecommand{\obs}{\phi} % function on each data point to get an observation
\providecommand{\aggregate}{\phi} % function on each data point to get
                                % an observation
\providecommand{\mdeg}{r} % degree of the moment matrix, currently i
                          % or r are the favored choices
\providecommand{\degree}[1]{\left|#1\right|}
\providecommand{\Sel}{\bS} % the selection matrix
\providecommand{\smono}[1]{{\left[#1\right]}}
\providecommand{\bUbasis}{\bU\smono{\bbeta_{1}; \ldots; \bbeta_{K}}}
\providecommand{\bUbasisshift}[1]{\bU\smono{\bbeta_{1} + \bgamma_{#1}; \ldots; \bbeta_{K} + \bgamma_{#1}}}
% indices and sizes

\providecommand{\monos}{\bv} % monomial basis
\providecommand{\monoss}{\mathcal{C}} % selected monomial basis

\providecommand{\cnstrfun}{g} % letter for the constraint function g = 
\providecommand{\cnstrfuns}{\boldsymbol{g}} % 
\providecommand{\cnstrfunname}{constraint function} % 

% talking about data
\providecommand{\XX}{\boldsymbol{X}} % P dimensional data
\providecommand{\ZZ}{Z} % latent variable 

\providecommand{\Multinomial}{\operatorname{Multinomial}}

%%%%  Terms %%%%%
% terms that might get renamed
\providecommand{\polymom}{Polymom} % name of the method
\providecommand\polymomprob{polymom problem} % name of the class of problem
                                % we want to solve
\providecommand{\MCP}{MCP} % moment completion problem
\providecommand{\GaMM}{Ga.M.M.} % 
\providecommand{\GeMM}{Gen.MM} % we talk about both Gaussian mixture and generalized method of mometns.
\providecommand{\tensordecomp}{tensor decomposition}
\providecommand{\tensorstruct}{special tensor structure}
\providecommand{\obsname}{observation function}
%%%%% problems %%%%
\providecommand{\feasibility}[2]{
  \begin{array}{cl}
    \textnormal{find} &{#1} \\
    \textnormal{s.t.}  &#2
  \end{array}
}

\providecommand{\minprob}[3]{
  \begin{array}{cl}
    \underset{#1}{\operatorname{minimize}}&{#2} \\
    \textnormal{s.t.}  &#3
  \end{array}
}

% linalg
\providecommand{\symmat}{\mathbf{S}} % \mS^k is space of symmetric k x k matrices
\providecommand{\tr}{\operatorname{tr}} % trace
\providecommand{\diag}{\operatorname{diag}}
\providecommand{\rank}{\operatorname{rank}}
\providecommand{\lspan}{\operatorname{span}}
\providecommand{\proj}{\operatorname{proj}}
\providecommand{\mpinv}{\dagger} % Moore-Penrose pseudoinverse superscript symbol
\providecommand{\nullity}{\operatorname{nullity}}
\providecommand{\T}{\mathsf{T}} % transpose
\providecommand{\vecs}{\operatorname{vecs}}
\providecommand{\colsp}{\operatorname{col}}
\providecommand{\nullsp}{\operatorname{null}}
\providecommand{\inv}{{-1}}

% misc.
\newcommand{\EE}{\mathbb{E}}
\newcommand{\indicator}[1]{\operatorname{\boldsymbol{1}}_{#1}}
\newcommand{\convergep}{\overset{p}{\to}}
\newcommand{\convergeas}{\overset{a.s}{\to}}
%\newcommand\eqdef{\ensuremath{\stackrel{\rm def}{=}}} % Equal bydefinition
\providecommand{\given}{\vert} % of (t) with additional stuff

% Editing notes
\forcecommand[2]{\editnote}{\ensuremath{\underline{\textrm{#1}}_{\textrm{#2}}}}
\forcecommand[1]{\editupnote}{\ensuremath{^{[\hl{\textrm{#1}}]}}}
\forcecommand{\vague}{\editupnote{vague}}
\forcecommand{\verify}{\editupnote{verify}}
\forcecommand{\reword}{\editupnote{reword}}
\forcecommand{\define}{\editupnote{define}}
\forcecommand{\expand}{\editupnote{expand}}
\forcecommand{\needcite}{\editupnote{citation needed}}
\forcecommand[1]{\findcite}{\editupnote{find: #1}}

% Referencing
\forcecommand[3]{\itemref}{\hyperref[#2:#3]{#1 \ref{#2:#3}}}
\forcecommand[1]{\sectionref}{\itemref{Section}{sec}{#1}}
\forcecommand[1]{\appendixref}{\itemref{Appendix}{sec}{#1}}
\forcecommand[1]{\algorithmref}{\itemref{Algorithm}{algo}{#1}}
\forcecommand[1]{\figureref}{\itemref{Figure}{fig}{#1}}
\forcecommand[1]{\tableref}{\itemref{Table}{tbl}{#1}}
\forcecommand[1]{\equationref}{\hyperref[eqn:#1]{Equation \ref{eqn:#1}}}
\forcecommand[1]{\problemref}{\hyperref[prob:#1]{Problem \ref{prob:#1}}}
\forcecommand[1]{\exampleref}{\hyperref[exa:#1]{Example \ref{exa:#1}}}


==> monomial.tex <==
\section{The monomial problem}
In this section, we consider the simplest case when the observed
moments are monomials of the parameters. We assume that $f_n(x)$ is
a monomial, the model is identifiable from the moments and all
possible monomial moments can be observed.  

Let $k$ be the number of mixture components and $d$ be the dimension
of the mixture model. The problem is to recover parameters $x_1, \ldots, x_k \in \Re^d$
and $\pi_1, \ldots, \pi_k \in \RR$ by observing moments of the form
$M_\alpha \eqdef \EE [X^{\alpha_i + \alpha_j}] =  \sum_{i=1}^k \pi_i x_i^\alpha$ where $\alpha \in
\NN^d$ is a vector of non-negative integers and
$x_i^\alpha \eqdef \prod_{j=1}^d x_{ij}^{\alpha_j}$.
For example, in the case of $d \geq k$, we know by the spectral
method that it is sufficient to observe moments where $|\alpha|_1 \eqdef
\sum_{j=1}^d \alpha_d \leq 3$. Another example is $d=1$, where it is sufficient
to observe $2k$ moments $M_0, \ldots M_{2k-1}$. We now
present a general algorithm that can solve both of these extremes and
intermediate problems.

\subsection{The multiplication matrix method}
Consider the vector of monomials $\theta(x) = [x^{\alpha_1}, \ldots, x^{\alpha_n}]$
of the $d$-dimensional variables $x$. 
(e.g. $\theta(x) = [x_1, x_2, \ldots, x_k, x_1^2, x_1 x_2, \ldots,
x_k^2, \ldots, x_1^3,  x_1^2 x_2, \ldots]$)
Our goal is to recover all $k$ vectors $\theta^{(1)}, \ldots, \theta^{(k)}$
for each mixture component. 
We would like to have enough monomials in $\theta(x)$,
so the vector of monomials $\phi_j(x) \eqdef x_j \theta(x)$
can be expressed as the same linear combination of $\theta$
at each of the $k$ true solutions.
That is, for any of the $k$ possible values of $x^*$
that generates our observed moments, we have

\begin{equation}
\label{eqn:mult}
\phi_j(x^*) = x^*_j \theta(x^*) = C_j \theta(x^*)
\end{equation}
for $C_j \in \RR^{n \times n}$. Let's call $C_j$ the multiplication matrix of the variable $x_j$.
Solving for $x_j$ is just an eigenvalue problem on $C_j$ if we can compute $C_j$.

Let $\Theta(x) \eqdef \theta(x) \theta(x)^\T$ be a $n \by n$ matrix and let
$\Phi_j(x) \eqdef x_j \Theta(x)$. 
By defintion $C_j \Theta(x^*) = \Phi_j(x^*)$.
Even though $\Theta(x)$ and $\Phi(x)$ are unknown,
some linear combination of them are exactly the observable moments!
Let $x^*_1, \ldots, x^*_k \in \RR^d$ be the true parameters,
then we can observe the following matrices
\begin{equation}
\hat{\Theta} \eqdef \sum_{i=1}^k \pi_i \Theta(x^*_i) \quad \textrm{and} \quad
\hat{\Phi}_j \eqdef \sum_{i=1}^k \pi_i \Phi_j(x^*_i) \quad \in \RR^{n \by n}
\end{equation}
where we also know that $\hat{\Theta}_{ij} = M_{\alpha_i + \alpha_j} = \EE[X^{\alpha_i+\alpha_j}]$.

Since the multiplication matrix applies termwise, we also know that
\begin{equation}
C_j \hat{\Theta} = \hat{\Phi}_j
\end{equation}

Now everything is simple if we can solve for $C_j$. Here are a few
examples where the basic algorithm applies.

\begin{example}[$d = 1$ any $k$]
This is the classical problem of recovering a univariate measure from
its moments where we observe the moments $\EE[X^p] = \sum_{i=1}^k \pi_i x_i^p$ for $p = 0,1,\ldots,2k-1$.
Pick $\theta(x) = [1, x^1, x^2, \ldots, x^{k-1}]$ then $\hat{\Theta}
\succeq 0$ is the Hankel matrix of moments of order 0 to
$2k-2$ which is invertible as long as all $x_i$'s are distinct. 
Solving for $C$ gives exactly the multiplication matrix! For $k=3$,
and  $\theta(x) = [1, x^1, x^2]$, we have
\begin{equation}
x \theta(x) = C \theta(x) = 
\begin{bmatrix}
 x \\ x^2 \\ x^3
 \end{bmatrix}
=
\begin{bmatrix}
 0 & 1 & 0 \\
 0 & 0 & 1 \\
 -c_0 & -c_1 & -c_2
 \end{bmatrix}
\begin{bmatrix}
 1 \\ x \\ x^2
 \end{bmatrix}
\end{equation}
Note that the last row states $x^3 + c_2 x^2 + c_1 x_1 + c_0 = 0$, and
these coefficients $c_i$ are unique given the 3 solutions of this cubic
equation.
\end{example}

\begin{example}[$d = k$]
\label{ex:spectral}
This is the class of problems solved by the spectral method. Suppose
we observe all second order moments $\EE[X_i X_j]$ and third order moments $\EE[X_i X_j X_k]$.
Pick $\theta(x) = [x_1, \ldots, x_k]$ then $\hat{\Theta} \succeq 0$ is
the matrix of second order moments, and $\hat{\Phi}_l$ is the
corresponding matrix of 3rd order moments with an extra $x_l$. When
the true parameters are linearly independent, $\hat{\Theta} \succ 0$
and is invertible. 
\end{example}

Note how example \ref{ex:spectral} did not require observing first order
moments. In contrast, we see in the following example how first order
moments can help.

\begin{example}[$d = k-1$]
As in example \ref{ex:spectral}, let's suppose we also observe $\EE[X_i]$.
Pick $\theta(x) = [1, x_1, x_2, \ldots, x_k]$ then $\hat{\Theta} \succeq 0$ is
the matrix of both first and second order moments. When
the true parameters plus the 1 vector are linearly independent, one can solve
for $C$. This can be done in general unless the parameters are inside
a subspace of smaller dimension.
\end{example}
Now two problems not addressed by the spectral method.

\begin{example}[$d = 2, k = 4$]
Pick $\theta(x) = [1, x_1, x_2, x_1 x_2]$, and the basic method would
require us to observe a 5th order moment $\EE[X_1^3 X_2^2]$. This
example illustrates how observing cross moments helps, since the case of
$d=1, k=4$  requires observing up to the 7th order moment.
\end{example}

Under our view, it is pretty clear what to do when spectral method does not
apply when $d \leq k$: we just add more, higher degree terms to the monomial
vector $\theta$ and observe more moments. In particular, we have the
following observation
\begin{prop}
If $k \leq 1+d+d^2+\ldots+d^p=\frac{d^{p+1}-1}{d-1}$, the basic problem is solvable by the
basic method if moments up to $2p+1^{th}$-order are observed and the 
corresponding vectors $\theta(x^*_1), \theta(x^*_2), \ldots,
\theta(x^*_k)$ of up to $p^{th}$ order moments are linearly
independent (true for random parameters?). 
\end{prop}



==> polynomial.tex <==
\section{The polynomial moment problem}
The case that the observed moments are monomials of the parameters
and that every required monomial is observed is quite
restrictive. Restrictive enough that even the Gaussian mixture is not covered.

Recall that our problem is to recover parameters $x_1, \ldots, x_k \in \RR^d$
and $\pi_1, \ldots, \pi_k \in \RR$ by observing moments of the form
$M_n =  \sum_{i=1}^k \pi_i f_n(x_i)$ where $f_1, \ldots, f_n$ are
polynomials of the parameters.

We will recover
all monomial moments from the observed moments and apply the basic
method to recover parameters. Our approach can be summarized as
follows
\begin{enumerate}
\item express observable moments over the distribution of the data
as polynomials of parameters
\item recognize this polynomial solving problem for mixture models as an
instance of the Generalized Problem of Moment where the underlying
measure to be recovered is on the parameters as opposed to a measure on the data.
\item solve the Generalized Problem of moment to get the
monomial moments
\item recover parameters using one of several possible solution
  recovery methods from monomial moments
\end{enumerate}


\subsection{Reduction to the Generalized Moment Problem}
We describe here how the polynomial solving problem corresponding to
mixture models is an
instance of the Generalized Problem of Moment that can be solved with
convex relaxations. 

\subsection{A convex optimization approach}

\subsection{the SDP relaxation}
\subsection{the LP relaxation}

\subsection{An algebraic approach}

